Observing LOD using Equivalent Set Graphs: it is mostly flat and sparsely linked

This paper presents an empirical study aiming at understanding the modeling style and the overall semantic structure of Linked Open Data. We observe how classes, properties and individuals are used in practice. We also investigate how hierarchies of concepts are structured, and how much they are linked. In addition to discussing the results, this paper contributes (i) a conceptual framework, including a set of metrics, which generalises over the observable constructs; (ii) an open source implementation that facilitates its application to other Linked Data knowledge graphs.

==> src_old/graph.tex <==
\paragraph{{\bf Graph compression}} aggregates clusters of nodes in order to obtain abstracted graphs with less, more informative, nodes. We define the notion of \emph{equivalence set graph} (cf. Section~\ref{sec:identysetgraph}), a compressed version of a knowledge graph such as LOD. Following a similar approach as in~\cite{Beek2018}, we create a set of \emph{affordable} procedures to build equivalence set graphs (cf. Section \ref{sec:algorithm}).

An \emph{equality set graph} is a graph in which nodes are equivalence classes (i.e. equality sets) of entities in a knowledge graph (i.e. classes, properties, individuals). The notion of equivalence, which determines the entities belonging to an equality set, is defined by the observer. For example, we may define that two entities belong to the same equality set only if they are related by \texttt{owl:equivalentClass}. In other cases, we may define that such relation must be \texttt{skos:exactMatch} or both (either in \emph{and} or \emph{or}). Edges in an equality set graph are \emph{specialisation} relations between equality sets. This relation is defined by the observer. For example, we may define that \texttt{skos:narrower} or \texttt{rdfs:subClassOf}, as specialisation relations.

%We built a data structure for facilitating the retrieval of all the entities that are \textit{implicitly} subsumed or equivalent to a class or a property.
%This data structure is a graph having collections of entities as nodes (called equivalence sets) and subsumption relations as edges.
%The idea is to compute a data structure for encoding a large hierarchy of classes and properties, thus providing Semantic Web practitioners with means for studying features of large hierarchies.
Since one would expect that the structure of a hierarchy is something that looks like a tree, where each node of the tree is a class or a property and each directed edge from a node to its a parent node denotes a subsumption.
However, as already observed in~\cite{Wang2006}, due to the multiple roots and cycles, hierarchies of classes and properties have not a tree shape.

Intuitively, every pair of entities within a node of the a graph is either explicitly or implicitly equivalent in the input dataset (i.e. LOD-a-lot in our study).
For example, given a class $c$, the explicitly equivalent entities of $c$ are all the entities $e$ such that  \texttt{<c,owl:equivalentClass,e>} and/or \texttt{<e,owl:equivalentClass,c>} is in the input dataset.
The entities that are implicitly equivalent to $c$ are all the entities $e$ connected to $c$ through a path of two or more occurrences of \texttt{owl:equivalentClass} or any other property that is transitively subsumed by or equivalent to \texttt{owl:equivalentClass}.

%If there exist an edge that connects a node $a=\{a_1,..,a_n\}$ with a node $b=\{b_1,...,b_m\}$, then there exists a entity $b_i \in b$ that is either explicitly or implicitly subsumed $a_j \in a$.

If an entity $b_i$ that belongs to a node $b$ is explicitly or implicitly subsumed by an entity $a_j$ that belongs to a node $a$, then there exists an edge from $b$ to $a$.
For example, given a class $c$, the entities explicitly subsumed by $c$ are all the entities $e$ such that  \texttt{<e,rdfs:subClassOf,c>} is in the input dataset.
The entities that are implicitly subsumed to $c$ are all the entities $e$ connected to $c$ through a path of two or more occurrences of  \texttt{rdfs:subClassOf} or any other property that is transitively subsumed by or equivalent to \texttt{rdfs:subClassOf}.

An example of equivalence set graph is provided in Figure~\ref{fig:example}.
In particular,  Figure~\ref{fig:output} depicts  the equivalence set graph computed from the input dataset of  Figure~\ref{fig:input}.
The graph contains four equivalence sets. 
The top node clearly represents the class \texttt{Agent} and encloses all the classes defining this concept in DOLCE (prefix \texttt{dul}) and W3C's Organization ontology (prefix \texttt{org}).
Three nodes inherit from \texttt{Agent}.
Two nodes come from DOLCE ontology (i.e. \texttt{dul:PhysicalAgent} and \texttt{dul:SocialAgent}).
The other node represent the class \texttt{Person} and contains the classes \texttt{dbo:Person}, \texttt{dul:Person} and \texttt{foaf:Person} that define what is a Person in the ontologies DOLCE, DBpedia ontology and FOAF.

\begin{figure}[t]
    \centering
    \begin{subfigure}[b]{0.48\textwidth}
        \includegraphics[width=\textwidth]{img/example1.pdf}
        \caption{Input}
        \label{fig:input}
    \end{subfigure}
    ~ %add desired spacing between images, e. g. ~, \quad, \qquad, \hfill etc. 
      %(or a blank line to force the subfigure onto a new line)
    \begin{subfigure}[b]{0.48\textwidth}
        \includegraphics[width=\textwidth]{img/example2.pdf}
        \caption{Output}
        \label{fig:output}
    \end{subfigure}
    \caption{Figure~\ref{fig:output} shows an equivalence set graph computed from input dataset of Figure~\ref{fig:input}.Prefixes \texttt{dul}, \texttt{org}, \texttt{dbo}, \texttt{foaf} are respectively associated to namespaces of ontologies: DOLCE, W3C's Organization, DBpedia ontology and FOAF.}\label{fig:example}
\end{figure}

The intuitions behind the equivalence set graph are formalised in the following definitions.
Definition~\ref{def:nodes}  specifies  entities within a node, Definition~\ref{def:edges} specifies  edges of the graph, whereas Definition~\ref{def:closure} is used by both previous definitions.


\begin{definition}[equivalence set]
    \label{def:nodes}
	Let $\mathcal{K}$ be a Knowledge Base\footnote{In this context a Knowledge Base can be considered as a set of triples.}, given an entity $e$ and an equivalence predicate $p_{eq}$ (for $e$), an equivalence predicate $p_e$ for $p_{eq}$ and a subsumption predicate $p_s$ for $p_{eq}$,  we define the \textbf{equivalence set} of e for the predicates $p_{eq}$, $p_e$ and $p_s$  (i.e. $\cl{I}{p_{eq}}{p_e,p_s}(e)$)  as the set of entities that are implicitly or explicitly stated as equivalent to e in $\mathcal{K}$ with respect to the predicate $p_{eq}$, i.e.:
	
	\[\cl{I}{p_{eq}}{p_e,p_s}(e)=\{ e_1| \exists p \in \cli{C}{p_e,p_s}{p_e,p_s}(p_{eq}). \langle e,p^+,e_1\rangle \in \mathcal{K}||\langle e_1,p^+,e\rangle \in \mathcal{K}\}\footnote{Note that $p^+$ indicates a  property path with one or more occurrences of a p.}\] 
	
	where $\cli{C}{p_e,p_s}{p_e,p_s}(p_{eq})$ is the closure of $p_{eq}$ with respect to predicates for equivalence (i.e. $p_e$) and subsumption (i.e. $p_s$), namely, the set of predicates that are  implicitly  equivalent to or subsumed by $p_{eq}$.
\end{definition}


\begin{definition}[Explicit/Implicit super equivalence sets]
    \label{def:edges}
	Let $\mathcal{K}$ be a Knowledge Base, given an equivalence set $\cl{I}{p_{eq}}{p_e,p_s}(e)$, an equivalence predicate $p_{eq}$ and a subsumption predicate $p_{sub}$  for entities in $\cl{I}{p_{eq}}{p_e,p_s}(e)$, a predicate for equivalence $p_e$ for $p_{sub}$ and a predicate for subusumption  $p_s$ for $p_{sub}$, we define the \textbf{explicit super set} of $\cl{I}{p_{eq}}{p_e,p_s}(e)$ for $p_{sub}$ (i.e. $\cl{H}{p_{eq},p_{sub}}{p_e,p_s}(\cl{I}{p_{eq}}{p_e,p_s}(e))$)  as the set of equivalence sets that contain at least one entity $e_1$ which explicitly subsumes e with respect to the predicate $p_{sub}$, i.e.:
	
	\[\cl{H}{p_{eq},p_{sub}}{p_e,p_s}(\cl{I}{p_{eq}}{p_e,p_s}(e))=\{\cl{I}{p_{eq}}{p_e,p_s}(e_1) | \exists e_1 \in \cl{I}{p_{eq}}{p_e,p_s}(e_1). \exists p \in  \cli{C}{p_e,p_s}{p_e,p_s}(p_{sub}). \langle e,p,e_1\rangle \in \mathcal{K} \}\]
	
	where $\cli{C}{p_e,p_s}{p_e,p_s}(p_{sub})$ is the closure of $p_{sub}$ with respect to predicate for equivalence (i.e. $p_e$) and subsumption (i.e. $p_s$).
	
	%\noindent
	%We define the \textbf{direct subset} of $\s{I}{p_{eq}}{p_e}{p_s}(e)$ for  $p_{sub}$ (i.e. $\si{S}{p_{sub}}{p'_e}{p'_s}(\s{I}{p_{eq}}{p_e}{p_s}(e))$)  as the set of equivalence sets that contain at least one entity $e_1$ which is explicitly subsumed by e with respect to the predicate $p_{sub}$, i.e.:
	
	%\[\si{S}{p_{sub}}{p'_e}{p'_s}(\s{I}{p_{eq}}{p_e}{p_s}(e))=\{\s{I}{p_{eq}}{p_e}{p_s}(e_1) | \exists e_1 \in \s{I}{p_{eq}}{p_e}{p_s}(e_1). \exists p \in  \mathcal{C}^-\substack{p'_e\\p'_s}(). <e_1,p,e> \in \mathcal{K}\}\]
	
	%where $\mathcal{C}^-\substack{p'_e\\p'_s}(p_{sub})$ is the closure of the inverse of  $p_{sub}$ with respect to the equivalence predicate $p'_e$ and the subsumption predicate $p'_s$.
	
	\noindent
    We define the \textbf{implicit super set} of $\cl{I}{p_{eq}}{p_e,p_s}(e)$ for $p_{sub}$ (i.e. $\clt{H}{p_{eq},p_{sub}}{p_e,p_s}(\cl{I}{p_{eq}}{p_e,p_s}(e))$)  as the set of equivalence sets that contain at least one entity $e_1$ which implicitly subsumes e with respect to the predicate $p_{sub}$, i.e.:
	
	\[\clt{H}{p_{eq},p_{sub}}{p_e,p_s}(\cl{I}{p_{eq}}{p_e,p_s}(e))=\{\cl{I}{p_{eq}}{p_e,p_s}(e_1) | \exists e_1 \in \cl{I}{p_{eq}}{p_e,p_s}(e_1). \exists p \in  \cli{C}{p_e,p_s}{p_e,p_s}(p_{sub}). \langle e,p^+,e_1\rangle  \in \mathcal{K} \}\]
	
	where $\cli{C}{p_e,p_s}{p_e,p_s}(p_{sub})$ is the closure of $p_{sub}$ with respect to the predicates for equivalence (i.e. $p_e$) and subsumption  (i.e. $p_s$).

\end{definition}
Formal definitions for both explicit (i.e. $\cli{H}{p_{eq},p_{sub}}{p_e,p_s}(\cl{I}{p_{eq}}{p_e,p_s}(e))$) and
implicit (i.e. $\clit{H}{p_{sub}}{p_e,p_s}(\cl{I}{p_{eq}}{p_e,p_s}(e))$) \textit{subsets} can be easily derived from the above ones by swapping $e$ and $e_1$ in the triples $\langle e,p,e_1\rangle$ and $\langle e,p^+,e_1\rangle$ and by substituting $\cli{C}{p_e,p_s}{p_e,p_s}(p_{sub})$ with $\cl{C}{p_e,p_s}{p_e,p_s}(p_{sub})$ (i.e. the closure of the inverse of  $p_{sub}$ with respect to the equivalence predicate $p_e$ and the subsumption predicate $p_s$).
It is worth noting that the definition of the \textit{explicit} super set is provided only for sake of clarity (since it is a special case of the implicit definition).


Intuitively, the closure for an entity e contains all the entities that are  either implicitly equivalent to e or implicitly subsumed by e.
\begin{definition}[Closure]
    \label{def:closure}
	
	Let $\mathcal{K}$ be a knowledge base, given an entity e, a predicate for equivalence $p_{eq}$ and a predicate for subsumption $p_{sub}$ for e, and a predicate for equivalence ($p_{e}$) and subsumption ($p_{s}$) for $p_{eq}$ and $p_{sub}$,
	we define the \textbf{closure} of e with respect to $p_{eq}$, $p_{sub}$, $p_{e}$ and $p_{s}$  (i.e.  $\cli{C}{p_{eq},p_{sub}}{p_{e},p_{s}}(e)$)  as the set of entities that are implicitly either  equivalent (w.r.t. $p_{eq}$ and  predicates in its closure)  to or subsumed (w.r.t. $p_{sub}$ and  predicates in its closure) by  e, i.e.:
	
	\[\cli{C}{p_{eq},p_{sub}}{p_{e},p_{s}}(e)=\{e_1 | e_1 \in \cl{I}{p_{e}}{p_e,p_s}(e) ||  e_1 \in  \cl{I}{p_{e}}{p_e,p_s}(e_1) \text{ such that } \cl{I}{p_{eq}}{p_e,p_s}(e_1) \in \clit{H}{p_{eq},p_{sub}}{p_e,p_s}(\cl{I}{p_{eq}}{p_e,p_s}(e)) \}\]

\end{definition}


The algorithm for computing equivalence set graphs is presented in Section~\ref{sec:algorithm}.
We compute two equivalence set graphs, one for classes and another for properties.
The analysis of these graphs is provided in Section~\ref{sec:stats}.

\subsection{Metrics}
{\bf Introduce: here we formally define the metrics informally described in Section \ref{}.}

\paragraph{\textbf{Size of properties and classes.}}
For each class $c$, we define the size of $c$ as the number of entities $e$ such that $\langle e, t, c\rangle$ where t is a predicate within the closure of \texttt{rdf:type} (i.e. $|\{t|t\in \cli{C}{p_{eq},p_{sub}}{p_e,p_s}(\texttt{rdf:type})\}|$).
For each property $p$, we define the size of $p$  as the number of triples having $p$ as predicate (i.e. $|\{\langle s, p, o\rangle |\langle s, p, o\rangle \in \mathcal{K}\}|$).

\paragraph{\textbf{Size of equivalence sets.}}
As for equivalence sets, we define two measures for estimating their size, called direct and indirect respectively.
The direct size of an equivalence set is defined as the sum of the size of entities within an equivalence set. 
The indirect size of an equivalence set is defined as the sum of direct size of the equivalence sets in its closure plus its direct size.
It is worth noticing that these measures do not take into account duplicates (e.g. an entity belonging to two different classes counts for two).

\paragraph{\textbf{Number of Black Nodes.}}
Blank nodes are anonymous RDF resources often used within ontologies to define class restrictions.
Although the usage of blank nodes is discouraged because they cannot externally referred, they are still widely used (according to~\cite{Mallea2011} $\sim$ 15\% of RDF nodes are blank nodes).
A blank node can be included in the if one of the following conditions holds.
\begin{enumerate*}[label=\textit{(\roman*)}]
    
    \item a class $c$ is defined equivalent to a class restriction (for example, representing the intersection of other two classes).
    In this case the blank node will be included in the equivalence set of $c$.
    
    \item a class $c$ is subsumed by a class restriction (for example, defining a cardinality constraint for the individuals of $c$).
    In this case the blank node will constitute a separate equivalence set which subsumes the set of $c$.
    
\end {enumerate*}
To evaluate the impact of blank nodes structure, we computed:
\begin{enumerate*}[label=\textit{(\roman*)}]
    \item the number of blank nodes within a graph;
    \item the number of equivalence sets containing only blank nodes;
    \item and, among these sets, those without instances.
\end{enumerate*}

\paragraph{\textbf{Maximum Height of a Node of the Graph.}}
We define as height of a node n of the graph the maximum distance (the number of traversed edges) between n and a sink of the graph (i.e. a node without outgoing edges, e.g. a root).



==> src_old/intro_val.tex <==
%The aim of the Semantic Web initiative is to create a Web in which data is expressed through a symbols with a shared syntax and semantics~\cite{Berners-Lee2001}.
%In this vision, machines  become capable of autonomously exchanging, analysing and using data found on the Web for their tasks, thus making the Web a huge knowledge base for intelligent agents. 
%In  the last 20 years research community, industry and public administration have contributed to make this vision true by giving birth to the Linked Open Data: a huge network of $\sim$200 billion\footnote{This estimation is obtained from metadata provided by \url{https://lod-cloud.net/}} linked facts formally and uniformly represented in RDF and OWL.

%The usual way in which applications interact with Linked Open Data (ideally) consists in selecting from LOD one or more datasets containing key information for their business, merging these datasets and accessing the merged dataset.
%Few examples applications envision the use of LOD without dataset boundary.
%The limited use of LOD (as a whole) can be ascribed to both a limited technological support for interacting (e.g. querying and reasoning at web scale etc.) with a huge amount of data and our limited understanding the structure of today's LOD.
%This situation makes hard to answer queries such as ``give me all (i.e. among those in a LOD dataset) the classes that are transitevely subsumed by \texttt{foaf:Person}'' or ''list all individuals that explicitly or implicitly belong to \texttt{org:Agent}''.

%In the last years tools like RDF-HDT~\cite{Fernandez2013} and crawls of the LOD like LOD-a-lot~\cite{Fernandez2017} enabled at querying large portions of the Web of data but the only  picture of LOD (as a whole) that we have is  provided by \url{lod-cloud.net}.
%This picture synthesizes LOD structure at dataset scale by giving an overview of  datasets published as Linked Open Data, the interlinking among these datasets and information about domain and dimension of datasets.
%The work done by \url{lod-cloud.net} is valuable but Semantic Web practitioners would benefit of a more fine-grained picture of  LOD cloud structure to enable an effective interaction with data.

%Over the years there have been several studies looking at LOD structure but only few of them provided tools for replicating the analysis over time and datasets for facilitating the interaction with LOD. 
%To this end we introduce a novel data structure, called identity set graph.
%An identity set graph is a graph in which nodes represent sets of equivalent entities (e.g. classes or properties) and  edges are subsumption relations among them.
%This data structure has multiple objectives: on the one hand it could serve for addressing common queries over Linked Data without enumerating all entities within a hierarchy (e.g. list all triples having p or a property transitively equivalent or subsumed by p); on the other this structure provide a fine grained picture (at entity-level) of LOD.
\todo[inline]{Check for terminology consistency through the whole paper: "identity set graph" becomes "equivalence set graphs"}

The collection of Linked Open Data (LOD) datasets forms the largest publically accessible Knowledge Graph (KG) that is available on the Web today.  Over the years, many studies have analysed these datasets, often focusing on the structure and dimension of the data, as well as providing statistics that shed light on the composition of the data (cf. Section~\ref{sec:related}).  In most cases, such observations have been based on relatively small samples of the LOD KG.  Moreover, it is not always clear how representative the chosen samples are.  This is especially the case when observations are based on one dataset(e.g., DBpedia), or a handful of datasets, draw from the much larger LOD KG.

Linked Open Data and Semantic Web ontologies are encoded using RDF facts and/or OWL axioms, thereby exhibiting a formal semantics.  Several analyses have sought to investigate how these formal languages are used in practice: how are certain formal constructs (e.g., \texttt{owl:sameAs} identity) used, and to what extent are LOD guidelines (e.g., limiting the use of blank nodes) followed in practice?

This paper presents observations that have been conducted across (a very large subject of) the LOD KG.  These observations are aimed at understanding how LOD ontologies are designed, thereby focusing on the use of classes and properties, together with their use in instance data.  Specifically, this paper provides new insights about (i) the number of concepts defined in LOD, (ii) the shape of ontological hierarchies, (iii) the extent to which recommended practices for ontology alignment are followed, and (iv) whether classes and properties are instantiated in a homogeneous way.  In other words, the overall the aim of this paper is to make detailed observations about the modeling \emph{style} of the LOD KG.  In addition to delivering the analysis itself, this paper describes the formalization and implementation of the used approach, thereby allowing similar large-scale analyses to be conducted by others.

In order to gain a clear picture of LOD ontologies, and in order to measure the above mentioned characteristics, we need to extract all classes and properties that are defined in todays LOD Cloud, and we need to compute the equivalence closure over these classes and properties.  This is not an easy task, since we must take into account the possibility that the standardized RDF and OWL primitives themselves (e.g. \texttt{rdf:type}, \texttt{rdfs:Class}, and \texttt{owl:equivalentTo}) are sometimes specialized by custom concepts.  For example, if a local ontology defines a class \texttt{:myClass} as \texttt{rdfs:subClassOf} \texttt{owl:Class}, we must extract all instances of \texttt{:myClass}.

It is very difficult to (a) reason over the whole LOD KG and (b) take these tricky details about semantic closures into account.  The long and short of it is that all contemporary reasoning and querying approaches fall short of allowing such large-scale and complex analyses to be conducted.  For this reason, we start out by formalizing the new notion of \emph{equivalence set graphs} that will help us reach the scale that we need in order to conduct our analyses.

Equivalence set graphs offer a compressed version of the LOD KG.  While a KG contains nodes, the ESG contains \emph{equivalence sets} of LOD entities, e.g. classes or properties, and its edges are specialisation relations, e.g. \texttt{rdf:subClassOf}, between them. For example, we may define an equivalence set graph $G$ for classes, where the nodes, i.e. equivalence sets, are defined by the \texttt{owl:equivalentClass} relation, and the edges between the nodes of $G$ are defined by \texttt{rdfs:subClassOf}. Let \texttt{:A}, \texttt{:B}, \texttt{:C} and \texttt{:D} be four classes, with \texttt{:A} equivalent to \texttt{:B}, \texttt{:A} subclass of \texttt{:C} and \texttt{:C} equivalent to \texttt{:D}. The resulting $G$ has two nodes $v_{1}$ and $v_{2}$ corresponding to two equivalence sets: one containing \texttt{:A} and \texttt{:B}, and the other containing \texttt{:C} and \texttt{:D}, respectively. Furthermore, $v_{1}$ has an edge towards $v_{2}$, carrying the semantics of \texttt{rdfs:subClassOf}.  
The concept of \emph{equivalence set graph} abstracts from classes and properties: it can be applied to support observations focusing on any KG entity, given a notion of equivalence and specialisation between them.

Equivalence set graphs provide many benefits over the raw KG when performing large-scale and complex semantic analyses.

For the purpose of our investigation, we build two equivalence set graphs, one for classes and one for properties.  By querying these graphs, we obtain a set of statistics on the dimension of LOD ontology entities.  Moreover, our observations show that there is lack of explicit linking (alignment) between ontological entities and that there is a significant number of concepts with empty extension.  Hierarchies of properties are mainly flat, while those of classes' have a varying degree depth, which can reach over 70 levels. 

Our approach has its limits and our observations provide a partial view as compared of what can be ideally observed in order to have a complete understanding of the actual modeling style of LOD ontologies. For example, we are unable to tell at the moment whether certain domains impact more than others on certain observation. For example, we may expect that biomedical ontologies have classes with empty extension....
Nevertheless, this work provides valuable insights on the current situation and put the basis for formulating additional research questions towards an understanding of how ontology engineering works in practice as well as possibly detecting areas of intervention, e.g. lack of support for facilitating ontology alignment. 

This paper makes the following contributions:

\begin{enumerate*}[label=\textit{(\roman*)}]
    \item It provides a detailed analysis of how classes and properties are used throughout the LOD KG.  The analysis is based on a very large subset of the LOD KG in order to be more representative that earlier research.
    \item It introduces the novel formal concept of \emph{equivalence set graphs}.  They offer a compressed version of a LOD KG, and facilitate the kind of analysis that is conducted in this paper.
    \item It presents an algorithm for computing equivalence set graphs for an arbitrary LOD KG.
    \item It provides a scalable and Open Source implementation of the algorithm, which allows others to compute equivalence set graphs for very large LOD KGs.
\end{enumerate*}

The structure of this paper is as follows:
\todo[inline]{Outline}


==> src_old/met.tex <==

The main procedure was first run on LOD-a-lot\footnote{LOD-a-lot, \url{http://lod-a-lot.lod.labs.vu.nl/}} for computing the hierarchy of identity sets of properties.
We excluded some annoying facts that we found on LOD-a-lot such as:
\begin{enumerate}
    \item rdf:type rdfs:subPropertyOf+ rdfs:subClassOf
    \item owl:equivalentClass rdfs:subPropertyOf+ rdfs:subPropertyOf
    \item rdfs:subClassOf rdfs:subPropertyOf+ rdfs:subPropertyOf
    \item rdf:type rdfs:subPropertyOf+ rdfs:subPropertyOf
\end{enumerate}
These facts are formally correct but mess the hierarchy up.
The procedure needed three cycles (c.f. line~\ref{line:mainloop} of the procedure~\ref{proc:main}) to reach the fixpoint.

From the hierarchy of predicates we computed the closure for the predicates \texttt{owl:equivalentClass}  and \texttt{rdfs:subClassOf}.
Then we computed the hierarchy of identity sets using the procedure~\ref{proc:classes}.
The datasets can be downloaded from \url{https://www.dropbox.com/s/1r3g9mlaehxh105/Archive.zip}

Results for classes:
\begin{itemize}
    
    \item Number of identity sets of classes: 3750108
    
    \item Maximum number of ontology classes within an identity set: 103993
    
    \item Number of properties contained in the closure of \texttt{owl:equivalentClass}: 2
    
    \item Number of properties contained in the closure of \texttt{rdfs:subClassOf}: 380
    
    \item Number of triples having the property contained in the closure of \texttt{owl:equivalentClass}: 1051979
    
    \item  Number of triples having the property contained in the closure of \texttt{rdfs:subClassOf}: 5573245
    
\end{itemize}

Results for properties:
\begin{itemize}
    
    \item Number of identity sets of properties: 96817
    
    \item Maximum number of ontology properties within an identity set: 11
    
    \item Number of properties contained in the closure of \texttt{owl:equivalentProperty}: 
    
    \item Number of properties contained in the closure of \texttt{rdfs:subPropertyOf}: 
    
    \item Number of triples having the property contained in the closure of \texttt{owl:equivalentProperty}: 
    
    \item  Number of triples having the property contained in the closure of \texttt{rdfs:subPropertyOf}: 
    
\end{itemize}

\subsection{Problems of Empirical Semantics}
\begin{minted}{turtle}
rdfs:subPropertyOf rdfs:domain        rdf:Property.       # W3C
rdfs:subClassOf    rdfs:domain        rdfs:Class.         # W3C
rdfs:subClassOf    rdfs:subPropertyOf rdfs:subPropertyOf. # BTC
\end{minted}

The third statement, which is part of the Billion Triple Challenge (BTC) dataset, turns all properties into classes.  This statement does not violate RDF(S) semantics, yet it does have far-reaching consequences for the entire Semantic Web, most of which are unwanted.

==> src_old/method.tex <==
%In order to assess to what extent LOD (as a whole) provides an empirical basis that can be used as background for knowledge-based tasks we started analysing LOD from its intentional level (i.e. its schema).
%The schema provides a picture of concepts and relations that one can find in a dataset thus describing data at an high level and offering an entry point to who intent to use that dataset.



\subsection{{Input source}} Ideally, our input is the whole Linked Open Data cloud (LOD), which is huge and distributed on the Web. To the best of our knowledge, LOD ontologies have never been analysed on a scale larger than $\sim$4B triples\todo{check this number}. One of the largest available dumps of LOD is provided by WebDataCommons\footnote{\url{http://webdatacommons.org}}~\cite{Meusel2014}, which in November 2018 crawled $\sim$31B triples. LOD-a-lot\footnote{\url{http://lod-a-lot.lod.labs.vu.nl/}}~\cite{Fernandez2017} contains $\sim$28B unique triples and it is the only resource that provides them as a single-dump file. For this reason we use LOD-a-lot as main source for our empirical analysis. 
%This work is the first attempt to compute the schema that emerges from LOD-a-lot.

LOD-a-lot contains only asserted triples, therefore a reasoning step is required to make sure that all relevant facts that can be inferred from them are included in our input source\footnote{For the sake of this study we are interested in computing the semantic closure of equivalence and subsumption relations between classes and properties.}. Reasoning over LOD-a-lot, considering its huge dimension, makes standard reasoners unsuitable. Other solutions, such as the use of clustering computing techniques (e.g.~\cite{Urbani2010}), require expensive resources both in terms of computational power and memory capacity. Although this is a possible way to go, a better approach would identify a way to efficiently compress LOD so as to reduce the scale of the computations. In the next Section we describe our proposal in this direction.


%We called this structure ``Identity Set Graph'' which is introduced in Section~\ref{sec:identysetgraph}.
%A common procedure for empirical tasks such as ours requires a reasoning step over the dataset before performing any observation so as to include all facts that can be inferred from the asserted triples. One of our aims is to develop a tool that enables to perform this task on standard laptops. Therefore, the dimension of LOD-a-lot makes the use of standard reasoners less than convenient. We also exclude other solutions such as the use of clustering computing techniques (e.g.~\cite{Urbani2010}), because of their expensive nature (both in terms of computational power and memory capacity). 


\subsection{Equivalence Set Graph}
\label{sec:identysetgraph}
\input{src/graph.tex}

\subsection{Metrics}
\label{sec:metrics}
\input{src/metrics.tex}



%\subsection{Identity Set Graphs from LOD-a-lot}
%\label{sec:stats}
%\input{src/lodGraph.tex}

==> src_old/objective.tex <==




\begin{itemize}
    \item {\bf Say what is the target of our observation: LOD emerging modeling style}
    \item {\bf Introduce an informal description of the measurements that we are going to perform and what we expect them to tell us: how many concepts are defined in LOD, how many of them as classes/properties, how much they are linked, how deep their hierarchies are, how big are their extensions, how many blank nodes are there, etc.} 
    \item {\bf Say that we want to build affordable tools, and a framework to enable performing similar analyses with minor effort}
\end{itemize}



==> src_old/side.tex <==
\begin{minted}{sparql}
# Query 1
SELECT DISTINCT ?class  WHERE {?class rdf:type owl:Class}

# Query 2
SELECT DISTINCT ?class  WHERE {
    _:resource 
        rdfs:subClassOf|owl:equivalentClass|owl:onClass|
        owl:someValuesFrom|rdfs:range|rdfs:domain|
        rdf:type 
    ?class}

# Query 3
SELECT DISTINCT ?class  WHERE {
	?class
	    rdfs:subClassOf|owl:equivalentClass|owl:disjointUnionOf|
	    owl:hasKey|owl:intersectionOf|owl:oneOf|owl:unionOf  
	_:resource .
}
\end{minted}
